Monocular Differentiable Rendering for Self-Supervised 3D Object Detection

3D object detection from monocular images is an ill-posed problem due to the projective entanglement of depth and scale. To overcome this ambiguity, we present a novel self-supervised method for textured 3D shape reconstruction and pose estimation of rigid objects with the help of strong shape priors and 2D instance masks. Our method predicts the 3D location and meshes of each object in an image using differentiable rendering and a self-supervised objective derived from a pretrained monocular depth estimation network. We use the KITTI 3D object detection dataset to evaluate the accuracy of the method. Experiments demonstrate that we can effectively use noisy monocular depth and differentiable rendering as an alternative to expensive 3D ground-truth labels or LiDAR information.

==> 04_implementation_details.tex <==
\section{Implementation Details}

\subsection{Training of Shape Generator}
We used ShapeNet~\cite{chang2015shapenet}

\subsection{System Configuration and Hyperparameters}
\label{subsec:exp:sysconfig}

All the experiments are performed on a cluster with 8 GPUs. 2D bounding boxes and instance segmentation masks are extracted with a pre-trained Mask R-CNN~\cite{he2017mask} model of X-152 in detectron2~\cite{wu2019detectron2}. The depth maps are extracted by a pre-trained PackNet~\cite{guizilini20193d}, a state-of-the-art monocular depth estimator that is trained with self-supervision. Hyperparameters are set to $\lambda_b = \lambda_m = \lambda_p = 1$, $\lambda_d = 0.2$, $\lambda_{dim} = 0.1$, and $t_b = 0.1$. We used Adam optimizer ~\cite{kingma2014adam} with $\alpha=0.03$, $\beta_1=0.5$, $\beta_2=0.9$ with the number of optimization iteration $150$. The hyperparameters for confidence weighting is set as $\alpha_m = 0.1$ and $\alpha_b = 0.03$.


==> 05_experiments_old.tex <==
\section{Experiments}
\label{sec:experiments}

We evaluate the proposed method on KITTI 3D~\cite{geiger2012we}, the most popular benchmark for 3D object detection in autonomous driving.

\subsubsection{Dataset}
\label{subsec:exp:dataset}
KITTI 3D dataset is composed of RGB images and LiDAR points, for which annotations of 2D bounding boxes, 3D object location, 3D object dimension, 1D object rotation angle along the {\it y}-axis are provided. Although most of the other monocular 3D detection methods use provided annotations for training, we do not use them at all. We also do not use LiDAR points in training and inference. We use the training and validation split proposed in~\cite{chen20153d}. We only focus on the {\it car} category as well as many other works~\cite{TODO}.

\subsubsection{Evaluation Metrics}
\label{subsec:exp:metrics}
Following a recent suggestion by~\cite{simonelli2019disentangling}, we use the $AP_{|R_{40}}$ metric that is currently used in the official KITTI benchmark leaderboard instead of the traditional $AP_{|R_{11}}$ metric. For reference, we provide evaluation and comparison using $AP_{|R_{11}}$ in the appendix.
Evaluation metrics are computed as follows. A 3D shape is projected onto the image plane, normalized with respect to the bounding box coordinates and the intersection-over-union (IoU) is computed. For the 3D location, we use the metric described in \footnote{TODO(dbeker): add paper}, given by the following formula:\footnote{TODO(dbeker): add formula}

\subsubsection{System Configuration}
\label{subsec:exp:sysconfig}

All the experiments are performed on a cluster with the following configuration: 2D bounding box and instance segmentation masks are extracted by a pre-trained Mask R-CNN~\cite{he2017mask} model of X-152 in detectron2~\cite{wu2019detectron2}, and depth maps are extracted by a pre-trained PackNet~\cite{guizilini20193d}, state-of-the-art of self-supervised monocular depth estimation. Hyperparameters are $\lambda_b = \lambda_m = \lambda_p = 1$, $\lambda_d = 0.2$, $\lambda_h = TODO$, $\lambda_{dim} = 0.1$, $t_b = 0.1$, and $t_m = 0.0$. Optimization is conducted using Adam optimizer~\cite{kingma2014adam} with $\alpha=0.03$, $\beta_1=0.5$, $\beta_2=0.9$ and the number of optimization iteration is set to $150$.

\subsection{Benchmark}
\label{subsec:exp:benchmark}

%%%%%%%% figure %%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t]
    \begin{center}
        \includegraphics[width=1.0\linewidth,bb=0 0 400 200]{./figure/figure1.pdf}
    \end{center}
    \caption{Representative results by our method. Input images with predicted 2D bounding boxes and instance masks, reconstructed images, and ground-truth (green) / predicted (red) 3D bounding boxes in bird's eye view (BEV) are shown. The white points in BEV indicates point clouds of instances generated by predicted depth maps.}
    \label{fig:result1}
\end{figure*}
%%%%%%%% figure %%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%% table %%%%%%%%%%%%%%%%%%%%%%%%
% Comparison with SOTA, AP40, validation set
\begin{table}[t]
    \small
    \begin{center}
        \begin{tabular}{l|c|ccc|ccc}
            \toprule
            \multirow{2}{*}{Method} & \multirow{2}{*}{Supervised} & \multicolumn{3}{c|}{3D detection} & \multicolumn{3}{c}{Bird’s eye view} \\ 
             ~ & ~ &  Easy & Moderate & Hard  & Easy & Moderate & Hard \\ 
            \midrule   
            MonoDIS~\cite{simonelli2019disentangling} & \checkmark & 11.06 & 7.60 & 6.37 & 18.45 & 12.58 & 10.66  \\
            MoVI-3D~\cite{simonelli2019single} & \checkmark & 14.28 & 11.13 & 9.68 & 22.36 & 17.87 & 15.73   \\
            \midrule     
            MonoDR                                     & & 12.32 & 7.33 & 5.39 & 19.93 & 12.17 & 8.97 \\
            \bottomrule
        \end{tabular}
    \end{center}
    \caption{Comparison of monocular 3D detection methods: Average Precision ($AP_{|R_{40}}$) on KITTI 3D {\it validation} set.}
    \label{table:val_ap40}
\end{table}
%%%%%%%% table %%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%% table %%%%%%%%%%%%%%%%%%%%%%%%
% Comparison with SOTA, AP40, test set
\begin{table}[t]
    \small
    \begin{center}
        \begin{tabular}{l|c|ccc|ccc}
            \toprule
            \multirow{2}{*}{Method} & \multirow{2}{*}{Supervised} & \multicolumn{3}{c|}{3D detection} & \multicolumn{3}{c}{Bird’s eye view} \\ 
             ~ & ~ &  Easy & Moderate & Hard  & Easy & Moderate & Hard \\ 
            \midrule   
            OFTNet & \checkmark & 1.61 & 1.32 & 1.00 & 7.16 & 5.69 & 4.61  \\
            FQNet & \checkmark & 2.77 & 1.51 & 1.01 & 5.40 & 3.23 & 2.46  \\
            ROI-10D & \checkmark & 4.32 & 2.02 & 1.46 & 9.78 & 4.91 & 3.74  \\
            GS3D & \checkmark & 4.47 & 2.90 & 2.47 & 8.41 & 6.08 & 4.94   \\
            MonoGRNet & \checkmark & 9.61 & 5.74 & 4.25 & 18.19 & 11.17 & 8.73   \\
            MonoDIS~\cite{simonelli2019disentangling} & \checkmark & 10.37 & 7.94 & 6.40 & 17.23 &13.19 & 11.12  \\
            SS3D & \checkmark & 10.78 & 7.68 & 6.51 & 16.33 & 11.52 & 9.93   \\
            M3D-RPN & \checkmark & 14.76 & 9.71 & 7.42 & 21.02 & 13.67 & 10.23 \\
            MoVI-3D~\cite{simonelli2019single} & \checkmark & 15.19 & 10.90 & 9.26 & 22.76 & 17.03 & 14.85   \\
            RMPL & \checkmark & 18.09 & 11.14 & 8.94 & 28.08 & 17.60 & 13.95  \\
            \midrule     
            MonoDR                                     & & TODO & TODO & TODO & TODO & TODO & TODO \\
            \bottomrule
        \end{tabular}
    \end{center}
    \caption{Comparison of monocular 3D detection methods: Average Precision ($AP_{|R_{40}}$) on KITTI 3D {\it test} set.}
    \label{table:test_ap40}
\end{table}
%%%%%%%% table %%%%%%%%%%%%%%%%%%%%%%%%

Fig.~\ref{fig:result1} shows representative results of monocular 3D detection by our method. We can understand that ours can detect 3D objects accurately nevertheless ours does not requires annotations about 3D objects for training. The upper result indicates that ours can estimate correct 3D location and rotation of objects even when the predicted depth map is noisy and unreliable. Though 3D localization of objects at far distance is difficult only from 2D image, in the bottom result, a correct location is recovered with the help of monocular depth estimation method.

Table~\ref{table:val_ap40} and Table~\ref{table:test_ap40} show quantitative valuation on {\it validation} set and {\it test} set, respectively. Scores of existing methods that do not use LiDAR data for training and inference are also shown. Surprisingly, the detection accuracy of ours are very well. It outperforms many recent methods that requires supervision for training, and comparable with state-of-the-art methods. This result indicates that supervised learning of 3D detection is generally difficult so far, and simple fitting-based methods are still promising thanks to the matured 2D object detection, instance segmentation, and self-supervised monocular depth estimation methods.

\subsection{Ablation Studies}
\label{subsec:exp:ablation}

%%%%%%%% table %%%%%%%%%%%%%%%%%%%%%%%%
% "Is depth needed?" 
% "What is a good way to integrate depth?"
\begin{table}[t]
    \small
    \begin{center}
        \begin{tabular}{c|c|ccc|ccc}
            \toprule
            \multirow{2}{*}{2D loss} & \multirow{2}{*}{Depth Integration} & \multicolumn{3}{c|}{3D detection} & \multicolumn{3}{c}{Bird’s eye view} \\ 
             ~ & ~ & Easy & Moderate & Hard  & Easy & Moderate & Hard \\ 
            \midrule   
             & As 2D depth map & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
             & As 3D point cloud & 0.10 & 0.10 & 0.04 & 0.75 & 0.57 & 0.50 \\
             & Both & 0.13 & 0.12 & 0.04 & 0.98 & 0.75 & 0.54 \\
            \checkmark & - & 4.82 & 2.88 & 1.91 & 7.96 & 4.96 & 3.64 \\
            \checkmark & As 2D depth map & 12.92 & 7.16 & 5.23 & 19.96 & 11.61 & 8.83 \\
            \checkmark & As 3D point cloud (Mihai) & 4.79 & 2.92 & 1.97 & 7.83 & 5.00 & 3.62 \\
            \checkmark & As 3D point cloud (Kato) & 5.01 & 2.91 & 1.90 & 7.77 & 4.86 & 3.58 \\
            \checkmark & Both & 12.32 & 7.33 & 5.39 & 19.93 & 12.17 & 8.97 \\
            \bottomrule

        \end{tabular}
    \end{center}
    \caption{Evaluation of 2D and 3D loss functions with different depth integration methods on KITTI 3D {\it validation} set.}
    \label{table:depth_integration}
\end{table}
%%%%%%%% table %%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%% table %%%%%%%%%%%%%%%%%%%%%%%%
% Is depth needed?
\begin{table*}[t]
    \small
    \begin{center}
        \begin{tabular}{c|ccc|ccc}
            \toprule
            \multirow{2}{*}{Point Registration Algorithm} & \multicolumn{3}{c|}{3D detection} & \multicolumn{3}{c}{Bird’s eye view} \\
             ~ & Easy & Moderate & Hard  & Easy & Moderate & Hard \\ 
            \midrule
            Vanilla ICP        & TODO & TODO & TODO & TODO & TODO & TODO \\
            Hausdorff Distance & 12.32 & 7.33 & 5.39 & 19.93 & 12.17 & 8.97 \\
            \bottomrule
        \end{tabular}
    \end{center}
    \caption{Effect of the registration algorithm on the accuracy: Average Precision ($AP_{loc}$) (in \%) on KITTI {\it validation} set.}
    \label{table:registration_performance}
\end{table*}
%%%%%%%% table %%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%% table %%%%%%%%%%%%%%%%%%%%%%%%
% Is depth needed?
\begin{table*}[t]
    \small
    \begin{center}
        \begin{tabular}{c|ccc|ccc}
            \toprule
            \multirow{2}{*}{Depth Network} & \multicolumn{3}{c|}{3D detection} & \multicolumn{3}{c}{Bird’s eye view} \\ 
             ~ & Easy & Moderate & Hard  & Easy & Moderate & Hard \\ 
            \midrule   
            GeoNet   & TODO & TODO & TODO & TODO & TODO & TODO \\
            GeoNet + PCN  & TODO & TODO & TODO & TODO & TODO & TODO \\
            PackNet  & 12.32 & 7.33 & 5.39 & 19.93 & 12.17 & 8.97 \\
            PackNet + PCN  & TODO & TODO & TODO & TODO & TODO & TODO \\
            LIDAR point clouds  & TODO & TODO & TODO & TODO & TODO & TODO \\
            \bottomrule
        \end{tabular}
    \end{center}
    \caption{Effect of the input depth on the accuracy: Average Precision ($AP_{loc}$) (in \%) of bird's eye view boxes on KITTI {\it validation} set.}
    \label{table:depth_networks}
\end{table*}
%%%%%%%% table %%%%%%%%%%%%%%%%%%%%%%%%

We combine 2D image reconstruction and 3D reconstruction using estimated depth. To confirm its effectiveness, we tested our method without 2D/3D loss functions. The results is shown in Table \ref{table:depth_integration}. When only 2D image reconstruction is considered as objective (seventh row vs fourth row), the accuracy significantly drops. This indicates the help of self-supervised depth is very important for our method. The performance drop of {\it Easy} objects is larger than {\it Hard} objects, which shows that depth is less reliable for object at far distances. This is probably because of the training loss function of self-supervised methods as pointed out by~\cite{you2019pseudo}, therefore introducing their proposed method would further improve the accuracy. Among two depth integration methods we proposed, while both are effective (fifth row and sixth row vs forth row), TODO is better (fifth row vs sixth row), and combining both further boosts accuracy (seventh row). When 2D reconstruction loss is not used, the accuracy is very poor (first to third rows), which demonstrates that 2D loss functions are indispensable.

Table~\ref{registration_performance} shows an evaluation of different point cloud matching method. TODO: add discussion when get results.

To study how the accuracy of pre-trained depth estimation networks affect to ours, we conducted another experiment. Table~\ref{depth_networks} shows detection accuracy with several pre-trained depth estimation networks. TODO: add discussion when get results.

Evaluation of other design choices are provided in the appendix.

\subsection{Limitations}
\label{subsec:exp:limitations}

%%%%%%%% figure %%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t]
    \begin{center}
        \includegraphics[width=1.0\linewidth,bb=0 0 400 200]{./figure/figure1.pdf}
    \end{center}
    \caption{Three major categories in that our method fails.}
    \label{fig:limitations}
\end{figure*}
%%%%%%%% figure %%%%%%%%%%%%%%%%%%%%%%%%

Image reconstruction of our method includes reconstruction of pixels, segmentation masks, and bounding boxes. Therefore, when segmentation masks or bounding boxes are not accurate, 3D localization based on them inevitably becomes inaccurate. The first row of Fig.~/ref{fig:limitations} shows this kind of error. Because a bounding box by the pre-trained model (Mask R-CNN) are not an {\it amodal} bounding box, it only bounds a visible part of cars. Therefore, fitting a reconstructed car into the bounding box fails, and 3D detection fails. This problem would be solved by fine-tuning the detector using a detection dataset with amodal bounding boxes. Actually, 2D detection accuracy of ours is not very good compared with recent 3D detection methods (see appendix).

Our system does not involve learning of location and rotation of objects. However, there are some cases that learning is essential. From the input image in the second row of Fig.~/ref{fig:limitations}, humans can easily understand arrangement of cars because humans have a learned knowledge about the relation of neighboring parked cars and their relation to a road. However, this inference cannot be done by our fitting-only approach. Combining ours with learning based methods would solve this problem.

In some cases, the model of image reconstruction is erroneous. For example, we assume that objects and the camera stand upright on the ground plane and they only have rotation along yaw axis. However, in the case of the third row in Fig.~/ref{fig:limitations}, this assumption does not hold.

Another weakness of ours is inference speed. Computation time is proportional to the number of detected objects, and the mean computation time per image on KITTI {\it validation} set is about one minute. As a unsupervised method, use ours as auto labeling and train a faster detector using estimated labels like~\cite{TODO} would be a practical solution.
